Time Series Learning using Monotonic Logical Properties

Cyber-physical systems of today are generating large volumes of time-series data. As manual inspection of such data is not tractable, the need for learning methods to help discover logical structure in the data has increased. We propose a logic-based framework that allows domain-specific knowledge to be embedded into formulas in a parametric logical specification over time-series data. The key idea is to then map a time series to a surface in the parameter space of the formula. Given this mapping, we identify the Hausdorff distance between boundaries as a natural distance metric between two time-series data under the lens of the parametric specification. This enables embedding non-trivial domain-specific knowledge into the distance metric and then using off-the-shelf machine learning tools to label the data. After labeling the data, we demonstrate how to extract a logical specification for each label. Finally, we showcase our technique on real world traffic data to learn classifiers/monitors for slow-downs and traffic jams.

==> sections/cpsgrader.tex <==
Massively Open Online Courses (MOOCs) present instructors the
opportunity to learn from a large amount of collected data to
automatically identify common correct solutions and mistakes.
Developing automatic grading systems for CyberPhysical System (CPS) MOOCs
using simulation presents a particularly unique challenge.
Juniwal et al.~\cite{juniwal2014cpsgrader} demonstrated a
semi-supervised procedure for a CPS MOOC that first used dynamic time
warping to cluster traces of student solutions, asked the instructor
to label representatives from the clusters, and then extracted a STL
formula from a PSTL template that characterized the
cluster. Vazquez-Chanlatte et al.~\cite{logicalClustering} provided an
unsupervised technique which used PSTL templates from
~\cite{juniwal2014cpsgrader} to induce a distance metric that
reproduced an arbitrarily chosen subset of the results
from~\cite{juniwal2014cpsgrader}. This distance metric required the
user to provide an {\em a priori\/} total ordering on the parameter
space which was used to select a single representative point on the
boundary of the validity domain.  Then for each signal, the distance
between representative points served as the distance metric for the
signals.
\begin{wrapfigure}{r}{0.4\textwidth}
  \centering
  \frame{\includegraphics[width=\linewidth]{imgs/obstacle_avoidance.pdf}}
  \caption{Cartoon illustration of the simulation task, where a robot
    bypasses an obstacle, and then reorients.}\label{fig:obstacle_avoidance}
\end{wrapfigure}
Thus, while the PSTL induced distance lessened the labeling
burden (since under the PSTL template, many superficially different
clusters become equivalent), the total orderings required a
fair amount of expertise to craft. In this experiment, we demonstrate
that simple PSTL templates along with the logical distance (Eq~\eqref{eq:logical_distance}) can be used to reproduce the results
of~\cite{juniwal2014cpsgrader} without labeled data and without an
{\em a priori\/} total ordering on the parameter space.
To illustrate, we focus on two tests centered around a simulated robot
interacting with an obstacle. The robot is expected to (i) collide with
the obstacle, (ii) bypass the obstacle, (iii) reorient to it's
pre-collision orientation, and (iv) continue moving in the pre-collision
orientation (see Fig~\ref{fig:obstacle_avoidance}). We use the
following two PSTL templates (derived
from~\cite{juniwal2014cpsgrader}) to characterize the obstacle
avoidance and reorientation phase respectively. Crucially, when
instantiated with particular parameters, these templates are
essentially the actual specification of the robot.
\begin{eqnarray}
  &\f_{avoid}(\tau_1, h_1) = \ev_{[0, \tau_1]}(pos.y < h_1)\\
  &\f_{reorient}(\tau_2, h_2) = \alw_{[0, 60 - \tau_2]}(pos.x \leq h_2)
\end{eqnarray}
Our goal is to develop a distance metric, where similar solutions and
failure modes are grouped together.
\begin{figure}[h]
  \begin{subfigure}[b]{0.59\textwidth}
    \centering
    \includegraphics[width=\linewidth]{imgs/cps_grader_demo_traces.png}
    \caption{Representative sample of student submissions for obstacle
      avoidance task. A correct submission will tend towards the
      bottom right corner.}\label{fig:obstacle_avoidance_demo}
  \end{subfigure}%
\hfill%
\begin{subfigure}[b]{0.39\textwidth}
  \centering
  \includegraphics[width=\linewidth]{imgs/avg_reorient_and_obstacle_avoid.png}
  \caption{Resulting pairwise distances and dendogram of the averaged
    logical distances of $\f_{avoid}$ and
    $\f_{reorient}$.}\label{fig:obstacle_avoidance_clusters}
\end{subfigure}
\end{figure}
Consider the representative sample of student submissions show in
Fig~\ref{fig:obstacle_avoidance_demo}.  Signal 0 shows a submission
that never moves. Signal 1 shows a submission that continually
collides with the obstacle. Signal 2 shows a submission that collides
with the obstacle and then slides around the obstacle as it attempts
to by bypass it. Signals 3 and 5 show two solutions going around the
obstacle in two different ways. Signal 4 shows a submission that
bypassed the obstacle, but failed to reorient.
The validity domain boundaries for $\f_{avoid}$ and $\f_{reorient}$
are shown in Fig~\ref{fig:obstacle_avoidance_boundaries} and
Fig~\ref{fig:reorient_boundaries} respectively.

\begin{figure}
  \centering
  \begin{subfigure}[b]{0.5\textwidth}
  \includegraphics[width=\textwidth]{imgs/obstacle_avoidance_boundaries.png}
  \caption{$\f_{avoid}$
    boundaries.\label{fig:obstacle_avoidance_boundaries}}
  \end{subfigure}%
  \begin{subfigure}[b]{0.5\textwidth}
  \includegraphics[width=\textwidth]{imgs/reorient_boundaries.png}
  \caption{$\f_{reorient}$ boundaries.\label{fig:reorient_boundaries}}
\end{subfigure}
\end{figure}


Observe that through
the lens of $\f_{avoid}$, the signals that avoid the obstacle (3, 4,
and 5) are correctly separated from signals the signals that do not
(0, 1, 2). Similarly, through the lens of the reorient template, the
signals that reorient (3,5) are separated from the signals that do not
reorient (0,1,2,4).

We averaged the logical distance (eq~\eqref{eq:logical_distance}) for
both templates yielding the adjacency matrix and dendogram shown in
Fig~\ref{fig:obstacle_avoidance_clusters}. Note that the first layer
of the dendogram separates solutions that correctly avoided the
obstacle. Within the avoided obstacle group, signals 3 and 5 are
correctly grouped together since they both reoriented.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../root"
%%% End:

